Symmetry-resolved dynamical purification in synthetic quantum matter

When a quantum system initialized in a product state is subjected to either coherent or incoherent dynamics, the entropy of any of its connected partitions generically increases as a function of time, signalling the inevitable spreading of (quantum) information throughout the system. Here, we show that, in the presence of continuous symmetries and under ubiquitous experimental conditions, symmetry-resolved information spreading is inhibited due to the competition of coherent and incoherent dynamics: in given quantum number sectors, entropy decreases as a function of time, signalling dynamical purification. Such dynamical purification bridges between two distinct short and intermediate time regimes, characterized by a log-volume and log-area entropy law, respectively. It is generic to symmetric quantum evolution, and as such occurs for different partition geometry and topology, and classes of (local) Liouville dynamics. We then develop a protocol to measure symmetry-resolved entropies and negativities in synthetic quantum systems based on the random unitary toolbox, and demonstrate the generality of dynamical purification using experimental data from trapped ion experiments [Brydges et al., Science 364, 260 (2019)]. Our work shows that symmetry plays a key role as a magnifying glass to characterize many-body dynamics in open quantum systems, and, in particular, in noisy-intermediate scale quantum devices.

==> ReplyScipost.tex <==
Ref 1:

We thank the Referee for their careful reading of the manuscript, and for the feedback. We have made an extra effort to correct a few remaining typos.

Ref 2: 

We thank the Referee for their careful reading of the manuscript, and for their comments, that we address below point by point. 

Point 1: 

Indeed, as pointed out by the Referee, we are considering a system where the dissipator shall satisfy weak symmetry: for instance, in our Bose-Hubbard model, the effect of a jump operator of the form $b^\dagger +b $ would not be captured by our theory. 

We have clarified this aspect in two parts of the manuscript:

a) at the beginning of Sec. 3.1, where the general conditions for the theory are presented (we have also included the references suggested by the Reviewer), where we have also emphasized that this choice reflects typical experimental conditions;

b) after Eq. 17, in a footnote we introduced.

In fact, dynamical purification can also occur even if weak symmetry is broken, as shown in our experimental example. Of course, in that case, the notion of entropy shall be handled with care, as the density matrix is not in block-diagonal form: still, symmetry resolved quantities have specific operational meaning even in that context, as we have elaborated upon in  Npj Quantum Inf. 7, 152 (2021) (in particular, the offer meaningful bounds to information witnesses). 

Point 2:

The Referee raises a very important point, partly connected to their third comment as well. Let us split the question into two parts - different sectors, and scaling of maximal purity.

A) In general, the principle that governs dynamical purification also applies to sectors that are not neighbors of the initially occupied one: first, dissipation scrambles information in the sector, and then, coherent dynamics partly re-order the latter. However, a clean mathematical understanding of this phenomenon is a non-trivial task. 

The reason is the following: while NN sectors can be rigorously treated with second order perturbation theory, going beyond this would require at least third order, or even higher orders in 1D (since tunneling is strongly limited). This seems, in principle, technically feasible: however, empirically, we found such effects to be quite small (one example is depicted in Fig. 7), so we decided not to focus on those, as they will likely have limited experimental applicability.  

B) Maximal purity: this is an extremely interesting question, that we had tried to address within out framework. Unfortunately, it turns out that the 'peak' region is something that, on its own, cannot be immediately captured by perturbation theory: it is exactly the timescale where states that belong to generic subspaces $E_2(-1), E_3(-1)$ become important, because of both (i) dynamics inside the partition and (ii) multiple dissipative events. Both of these effects are well beyond our theory, so we are unable to capture neither the position nor the maximum of the peak with precision. We are only able to determine the scaling functions (see Eq. 23). Empirically, we have observed that the position of the maximum seems relatively unaffected by noise and even interactions in both XY, Bose-Hubbard, and U(1) lattice gauge theories (Fig. 4, 5, 6), so this may suggest some generic scaling, but as it stands, this shall be understood as a numerical observation. 

Point 3: 

We have added the population dynamics also for some sample cases of our simulations (most models follow the same pattern) with a new appendix including 3 figures, spanning several parameter regimes. We have also commented that, in the regime of dynamical purification, the probability of being in a sector that is neighbor to the starting one is expected to grow linearly with time, and then enter a quadratic regime, similarly to the prefactors $A(t)$.



Ref 3:

We thank the Referee for their careful reading of the manuscript, and for the positive assessment. We have included the paper suggested to our bibliography together with the previously cited review article.
